TART: An Open-Source Tool-Augmented Framework for Explainable Table-based Reasoning

Current Large Language Models (LLMs) exhibit limited ability to understand table structures and to apply precise numerical reasoning, which is crucial for tasks such as table question answering (TQA) and table-based fact verification (TFV). To address these challenges, we introduce our Tool-Augmented Reasoning framework for Tables (TART), which integrates LLMs with specialized tools. TART contains three key components: a table formatter to ensure accurate data representation, a tool maker to develop specific computational tools, and an explanation generator to maintain explainability. We also present the TOOLTAB dataset, a new benchmark designed specifically for training LLMs in table-tool integration. Our experiments indicate that TART achieves substantial improvements over existing methods (e.g., Chain-of-Thought) by improving both the precision of data processing and the clarity of the reasoning process. Notably, TART paired with CodeLlama achieves 90.0% of the accuracy of the closed-sourced LLM GPT-3.5-turbo, highlighting its robustness in diverse real-world scenarios. All the code and data are available at https://github.com/XinyuanLu00/TART.

==> figures/ood.tex <==
% \begin{figure}[!ht]
%     \centering
%     \begin{tikzpicture}[scale=0.6]
%     \small{
%         \begin{axis}[
%                 ymajorgrids,
%                 xmajorgrids,
%                 grid style=dashed,
%                 ybar=3pt,
%                 bar width=0.8cm,
%                 enlarge x limits=0.2,
%                 width=.7\textwidth,
%                 height=.4\textwidth,
%                 symbolic x coords={ TATQA,WikiTableQuestion,HiTab, HybridQA},
%                 xtick={HiTab, WikiTableQuestion, TATQA, HybridQA},
%                 ytick={0,10,...,70},
%                 nodes near coords,
%                 every node near coord/.append style={font=\small},
%                 nodes near coords align={vertical},
%                 ymin=0, ymax=70,
%                 ylabel={Accuracy},
%                 xlabel={Datasets}
%             ]
%              \addplot[blue, fill=blue!20, bar shift=0pt, text=black] coordinates {
%                                 (HybridQA, 60.9)
%                                 (HiTab, 46.0)
%                 (WikiTableQuestion, 42.9)
%                 (TATQA, 13.9)
%              };
%         \end{axis}
%     }
%     \end{tikzpicture}
%     \caption{Results on OOD datasets}
%     \label{fig:ood}
% \end{figure}

\begin{figure}[!ht]
    \centering
    \begin{tikzpicture}[scale=0.6] % Adjust scale to make the figure fit within one column
    \small{
        \begin{axis}[
                ymajorgrids,
                xmajorgrids,
                grid style=dashed,
                ybar=3pt,
                bar width=0.45cm, % Wider bars
                enlarge x limits=0.2,
                width=.8\textwidth, % Adjust width
                height=.5\textwidth, % Adjust height
                symbolic x coords={HybridQA, HiTab, WikiTableQuestion, TATQA}, % Reordered datasets
                xtick=data,
                ytick={0,10,...,90}, % Increased ymax
                nodes near coords,
                every node near coord/.append style={font=\footnotesize, color=black, yshift=2pt}, % Set font color to black, move labels up
                nodes near coords align={vertical},
                ymin=0, ymax=90, % Increased ymax to fit all values
                ylabel={Accuracy},
                xlabel={Datasets},
                legend style={at={(1,1)}, anchor=north east, legend columns=1}, % Legend location at top right inside the chart
            ]
             \addplot[blue, fill=blue!40, postaction={pattern=north east lines}] coordinates {
                (HybridQA,77.8) (HiTab,10.4) (WikiTableQuestion,22.1) (TATQA,6.3)
             };
             \addlegendentry{TART Llama2-7b}

             \addplot[red, fill=red!30, postaction={pattern=north west lines}] coordinates {
                (HybridQA,69.1) (HiTab,36.5) (WikiTableQuestion,38.5) (TATQA,5.0)
             };
             \addlegendentry{TART \small{Llama3-8b}}

             \addplot[green, fill=green!20, postaction={pattern=crosshatch dots}] coordinates {
                (HybridQA,66.7) (HiTab,34.4) (WikiTableQuestion,36.5) (TATQA,7.3)
             };
             \addlegendentry{TART Codellama-7b}

             \addplot[yellow, fill=yellow!20, postaction={pattern=crosshatch}] coordinates {
                (HybridQA,61.1) (HiTab,49.2) (WikiTableQuestion,39.4) (TATQA,9.5)
             };
             \addlegendentry{TART DeepSeek-7b}
        \end{axis}
    }
    \end{tikzpicture}
    \caption{Results on OOD datasets for different models}
    \label{fig:ood}
\end{figure}



